Average-case Complexity of Teaching Convex Polytopes via Halfspace Queries

We examine the task of locating a target region among those induced by intersections of $n$ halfspaces in $\mathbb{R}^d$. This generic task connects to fundamental machine learning problems, such as training a perceptron and learning a $\phi$-separable dichotomy. We investigate the average teaching complexity of the task, i.e., the minimal number of samples (halfspace queries) required by a teacher to help a version-space learner in locating a randomly selected target. As our main result, we show that the average-case teaching complexity is $\Theta(d)$, which is in sharp contrast to the worst-case teaching complexity of $\Theta(n)$. If instead, we consider the average-case learning complexity, the bounds have a dependency on $n$ as $\Theta(n)$ for \tt{i.i.d.} queries and $\Theta(d \log(n))$ for actively chosen queries by the learner. Our proof techniques are based on novel insights from computational geometry, which allow us to count the number of convex polytopes and faces in a Euclidean space depending on the arrangement of halfspaces. Our insights allow us to establish a tight bound on the average-case complexity for $\phi$-separable dichotomies, which generalizes the known $\mathcal{O}(d)$ bound on the average number of "extreme patterns" in the classical computational geometry literature (Cover, 1965).

==> 5.halfspace_ranking.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Teaching Ranking via Pairwise Comparisons}\label{sec.applied.ranking}
In this subsection, we consider the task of finding the ranking over a set of objects embedded in $\Rd$ in general position (see \defref{general position vectors}). A ranking over a set of $n$ objects $\Theta = \curlybracket{\theta_1,\theta_2,\cdots,\theta_n}$ is an ordering $\sigma: \bracket{n} \rightarrow \bracket{n}$ of the form:
$\sigma\parenb{\Theta}:= \theta_{\sigma(1)} \prec \theta_{\sigma(2)}\cdots \prec \theta_{\sigma(n-1)} \prec \theta_{\sigma(n)}$.
We assume that for any ranking $\sigma$, there is a \tt{reference point} $r_{\sigma}$ such that if $\sigma$ ranks $\theta_i \prec \theta_j$ , then $||\theta_i - r_{\sigma}|| < ||\theta_j - r_{\sigma}||$. We refer to such assumption as {\bf E1}---This leads to an interpretation of a query ``is $\theta_i$ closer to $r_{\sigma}$ than $\theta_j$'', as identifying which side of the bisecting hyperplane of $\theta_i$ and $\theta_j$ does $r_{\sigma}$ lies in (as shown in \figref{fig:example.ranking}). 
\begin{definition}[Bisecting hyperplane]\label{bisecting hyperplane}
A hyperplane $h_{i,j}$ in $\Rd$ is a bisecting hyperplane to objects $\theta_i$ and $\theta_j$ if both are equidistant from $h_{i,j}$ and $h_{i,j}\cdot (\theta_i - \theta_j) = 0$.
\end{definition}
Thus, $n$ objects lead to $\binom{n}{2}$ hyperplanes (one query for each pair of objects) in $\Rd$:\\
$\underbrace{n\: \textnormal{embedded objects in\:} \Rd}_{\textnormal{Rankings of\:} \Theta}
    \stackrel{\boldsymbol{\textbf{E1}}}{\:\leadsto\:} \underbrace{ {\tiny \binom{n}{2}} \textnormal{ hyperplanes in\:} \Rd}_{\textnormal{Convex polytopes : reference points}}$
Each convex polytope corresponds to a reference point, thereby to a ranking of objects.
\paragraph{Teaching rankings as teaching convex polytopes} Denote the $\binom{n}{2}$ hyperplanes induced by pairwise-comparison of $n$ embedded objects by $\Hndp$.
Following our teaching framework in \secref{section: teaching framework}, we know that $\regionpair$ induced by $\cA(\Hndp)$ forms the underlying hypothesis class; with instances $\Hndp$ and corresponding labeling set $\{1,-1\}$. Thus, teaching a ranking $r_{\sigma}$ corresponds to providing the teaching set $\mathcal{TS}(\Hndp,r_{\sigma})$ to a learner.

Interestingly, we note that 
the hyperplanes induced by pairwise comparison of objects are no longer in general position. For example, in \figref{fig:example.ranking}, the three bisecting hyperplanes induced by any three points (in $\reals^2$) intersect at an 1-d subspace.
The following result, proved in \iftoggle{longversion}{\appref{appendix: teaching ranking}}{the supplemental materials}, shows that even under this special arrangement of hyperplanes, the average complexity for teaching such a ranking is $\bigTheta{d}$.
\begin{theorem}\label{theorem: teaching ranking}
Assume $\bf{E1}$ and $r_{\sigma}$ $\sim$ $\mathcal{U}$. There exists a teaching algorithm which requests $\bigTheta{d}$ pairwise comparisons on average for ranking \tt{i.e.} $\mathbb{E}_{\mathcal{U}}[M_n] = \bigTheta{d}$ where $M_n$ denotes a random variable for the number of pairwise
comparisons requested by an algorithm. In other words, the average teaching complexity of ranking via pairwise comparisons is $\bigTheta{d}$.
\end{theorem}
The above average complexity bound is achievable by running a variant of \algoref{algo: teaching halfspace} (\secref{subsection: main theorem}) where for a uniformly random ranking $r_{\sigma}$, teacher provides the halfspace queries corresponding to $\mathcal{TS}(\Hndp,r_{\sigma})$ in each iteration. To prove \thmref{theorem: teaching ranking} we draw insights from 
\secref{subsection: main theorem}, in particular \eqnref{eqn:tag:a.2}. We denote the number of regions $\fr\parenb{\cA(\Hndp)}$ as $C(n,d)$.
Equivalent to \thmref{thm:d'-general} and \propref{faces_teach},
we show that the number of regions and faces could be bounded by analyzing the recursion:  $C(n,d) = C(n-1,d) + C(n-1,d-1)$  \cite{jamieson2011active}. We further bound the ratio $\ff\parenb{\cA(\Hndp)}\boldsymbol{/}\fr\parenb{\cA(\Hndp)}$ between constant factors of $d$, which gives $\bigTheta{d}$ on the average teaching complexity of ranking.

==> abstract.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
%\looseness-1
We examine the task of locating a target region among those induced by intersections of $n$ halfspaces in $\mathbb{R}^d$. This generic task connects to  fundamental machine learning problems, such as training a perceptron and learning a $\phi$-separable dichotomy. We investigate the \emph{average teaching} complexity of the task, i.e., the minimal number of samples (halfspace queries) required by a \emph{teacher} to help a version-space learner in locating a \emph{randomly} selected target. As our main result, we show that the average-case teaching complexity is  $\Theta(d)$, which is in sharp contrast to the worst-case teaching complexity of $\Theta(n)$. If instead, we consider the average-case learning complexity, the bounds have a dependency on $n$ as $\Theta(n)$ for \tt{i.i.d.} queries and $\Theta(d \log(n))$ for actively chosen queries by the learner. Our proof techniques are based on novel insights from computational geometry, which allow us to count the number of convex polytopes and faces in a Euclidean space depending on the arrangement of halfspaces. Our insights allow us to establish a tight bound on the average-case complexity for $\phi$-separable dichotomies, which generalizes the known $\mathcal{O}(d)$ 
bound on the average number of ``extreme patterns'' in the classical computational geometry literature (Cover, 1965).

%We examine the task of locating a target region among those induced by intersections of $n$ halfspaces in $\mathbb{R}^d$. This generic task connects to several fundamental problems in machine learning, including the problem of training a perceptron and learning a $\phi$-separable dichotomy. \yuxin{needs to rephrase this considering that we no longer discuss ranking and that $\phi$-separable dichotomy could be considered as a more general case. ``several fundamental problem'' does seem to be proper here}\akash{Right. We should remove several. Maybe we can rephrase ``connects to the fundamental machine learning problems of training a perceptron and learning a $\phi$-separable dichotomy''} %and finding a ranking function over a set of objects via comparison queries. 
%We investigate the \emph{average teaching} complexity of the task, i.e., the minimal number of samples (halfspace queries) required by a \emph{teacher} to help a version-space learner in locating a \emph{randomly} selected target. As our main result, we show that the average-case teaching complexity is  $\Theta(d)$\akash{$\Theta(d')$, should point out Fukuda here?}\yuxin{i think including $d'$ and Fukuda in abstract is too much -- let's do it in the bullet points in intro}\akash{how do we differentiate Fukuda with $\Theta(d)$?}, which is in sharp contrast to the worst-case teaching complexity of $\Theta(n)$. If instead, we consider the average-case learning complexity, the bounds have a dependency on $n$ as $\Theta(n)$ for \tt{i.i.d.} queries and $\Theta(d \log(n))$ for actively chosen queries by the learner. Our proof techniques are based on novel insights from computational geometry, which allow us to count the number of convex polytopes and faces in a Euclidean space depending on the arrangement of halfspaces. Our insights allows us to establish a tight bound on the average-case complexity for $\phi$-separable dichotomies, which recovers the known $\mathcal{O}(d)$ \akash{in addition to showing $\bigO{d'}$ on extreme points?} \yuxin{how about ``which generalizes the known ...'', rather than specifying $d'$ here?}\akash{works} bound on the average number of ``extreme patterns'' in the classical computational geometry literature \citet{cover1965geometrical} \yuxin{text cite}\akash{natbib is not working}
%Building on our techniques, we provide the following results: (i) when teaching a ranking function induced by distances of objects $\mathrm{wrt}$ a reference point in a Euclidean space, we establish a new bound of $\Theta(d)$ average-case teaching complexity, and (ii) when teaching $\phi$-separable dichotomies, we recover the known $\mathcal{O}(d)$ bound on the average number of ``extreme patterns'' in the classical computational geometry literature \cite{cover1965geometrical}.
\end{abstract}

==> analysis.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> learning.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\clearpage
\section{Connections to Learning Complexity}\label{sec.learning}
In this section, we consider the problem of learning a convex polytope via halfspace queries, \emph{without} the presence of a helpful teacher. We consider both the passive learning setting where learner makes \emph{i.i.d.} queries and the active learning setting with actively chosen queries, and provide sample complexity results accordingly.
\vspace{-2mm}
\paragraph{Learning convex polytopes via halfspace queries} Consider the hyperplane set $\Hnd$ in $\Rd$ and a target region $r^* \in \regionset$. For any hyperplane $h \in \Hnd$
where $h = \condcurlybracket{\h{}}{\eta_h \cdot \h{}= b_h,\: \h{}\in \mathbb{R}^d}$, the labeling function $\ell_{r^*}$, as defined in \secref{sec.formulation}, specifies its label (halfspace) as $\ell_{r^*}(h) = $ $\mathrm{sgn}\parenb{\eta_h \cdot r^*- b_h}$ .
The problem of learning a region $r^*$ therefore reduces to identifying the corresponding labeling function $\ell_{r^*}$.
The objective here is to learn the region by querying the reference
of the form
    $q_{h}:= \mathbf{1}\curlybracket{\ell_{r^*}(h) = 1}$,
where $h \in \Hnd$ and $\mathbf{1}\curlybracket{\cdot}$ is the indicator function. 
Similar to the teaching setting, we assume that the target $\rgn^*$ is sampled uniformly at random. 
In the following two subsections, we establish sample complexity results, i.e., on the minimal number of halfspace queries required to determine a target region, under the settings of \tt{active} and \tt{passive} learning.

\subsection{Active learning of convex polytopes}\label{sec:active learning}

In subsection \secref{subsection: main theorem}, we showed that worst-case teaching complexity for convex polytopes is $\bigOmega{n}$,  
this directly implies the lower bound of $\bigOmega{n}$ on the worst-case for active learning.
In the following, we show that when the underlying hyperplane arrangement is in \gen{}, the average-case complexity of active learning has only a $\log n$ dependency on the number of hyperplanes. 

We achieve this by actively selecting 
informative (ambiguous) queries---a similar characterization of the ambiguous queries as considered by \citet{jamieson2011active} for the pairwise ranking problem.
Concretely, we consider the following
querying strategy: For an (unknown) target region $\rgn$ $\in \regionset$  and a uniformly random ordering of hyperplanes $\Hnd$, the (active) learner checks in each iteration if a query $q_{h}$  is ambiguous for randomly selected $h \in \Hnd$ (i.e. intersects the convex body defined by hyperplanes sampled previously); then asks or imputes the labels depending on their ambiguity.\\
\newline
In any iteration $k$ of the above query selection procedure, denote the event of requesting the query for a sampled hyperplane $h^{(k)}$ by $B_k$. That is, $B_k = {\bf 1}\curlybracket{q_{h^{(k)}} \text{is requested}}$. Note that each $B_k$ is a Bernoulli distribution with \tt{unknown} parameter $(\star)$ to be ascertained. If we can bound $(\star)$ then we bound the expected number of queries as well. For a  size $k$ subset $\mathcal{S} \subseteq \Hnd$, we notice that the $(k+1)^{\mathrm{th}}$ sampled hyperplane is ambiguous if it intersects the convex body defined by hyperplanes in $\mathcal{S}$. Thus we want to bound the probability of the event that the query $q_{h^{(k+1)}}$ is ambiguous. Denote the probability of such an event as $P_A(k,d,\mathcal{U})$. Notice $P_A(k,d,\mathcal{U})$ is our $(\star)$ here. In \lemref{probability ambiguity hyperplane}, we show that $P_A(k,d,\mathcal{U})$ is upper bounded by a factor of $1/k$ for relatively small sample size $k$. 
\begin{lemma}[Probability of ambiguity]\label{probability ambiguity hyperplane}
 Assume  $\rgn \sim \mathcal{U}$. Let $P_A(k, d, \mathcal{U})$ denote the probability of the event that the query $q_{h^{(k+1)}}$ is ambiguous where $h^{(k+1)}$ is the $(k+1)^{\mathrm{th}}$ sampled hyperplane. If $\Hnd$ is in $d'$-relaxed general position, then there exists a positive, real
number constant $a$ independent of $k$ such that for $k > 2d'$, $P_A(k, d, \mathcal{U}) \le a\cdot\frac{d'}{k}$.
\end{lemma}
\lemref{probability ambiguity hyperplane} allows us to bound the expected value of $\sum_{j=1}^n {\bf 1}\{q_{h^{(j)}}\text{is requested}\}$. As detailed in \iftoggle{longversion}{\appref{appendix: active learning}}
{the supplemental materials}, we show that for hyperplane arrangement in $d'$-relaxed general configuration, the expected value for $\sum_{j=1}^n {\bf 1}\{q_{h^{(j)}}\text{is requested}\}$ is $\bigTheta{d'\log n}$. 
This leads to the following complexity results for active learning (proofs are provided in \iftoggle{longversion}{the Appendix}{the supplemental materials}). 
\begin{theorem}\label{pairwise teaching bound}
Assume $\rgn$ $\sim$ $\mathcal{U}$ and that the underlying hyperplane arrangement of $\Hnd$ is in $d'$-relaxed general position.
Let
$M_n$ denote a random variable for the number of queries that are requested in the query selection procedure in \secref{sec:active learning}, then $\mathbb{E}_{\mathcal{U}}[M_n] = \bigTheta{d'\log n}$,
\tt{i.e.} the average-case query complexity of convex polytopes is $\bigTheta{d'\log n}$.
Moreover, the worst-case query complexity is $\bigTheta{n}$.
\end{theorem}
\subsection{Passive learning of convex polytopes} 
In the case of passive learning of a target region, the \tt{average} sample complexity is trivially lower bounded by $\bigOmega{n}$ since the learner gets a label uniform at random. Thus, on average it requires to sample $n$ times to reconstruct the labels for all the halfspaces corresponding to the enclosing hyperplanes. Since there are $n$ hyperplanes $n$ samplings are sufficient to get all the labels which trivially give a $\cO(n)$ solution. Thus, it is not very difficult to see that in the case of passive learning the average sample complexity is $\bigTheta{n}$. 


==> learning_subsection_old_content.tex <==
\subsection{Connection to average-case learning complexity}\label{subsec: connection to learning}
In this subsection, we consider learning a convex polytope via halfspace queries in absence of a teacher. We consider both the passive learning setting where learner makes \emph{i.i.d.} queries and the active learning setting with actively chosen queries, and provide sample complexity results accordingly.

\paragraph{Learning convex polytopes via halfspace queries} Consider the hyperplane set $\Hnd$ in $\Rd$ and a target region $r^* \in \regionset$. For any hyperplane $h \in \Hnd$
where $h = \condcurlybracket{\h{}}{\eta_h \cdot \h{}= b_h,\: \h{}\in \mathbb{R}^d}$, the labeling function $\ell_{r^*}$, as defined in \secref{sec:formulation}, specifies its label (halfspace) as $\ell_{r^*}(h) = $ $\mathrm{sgn}\parenb{\eta_h \cdot r^*- b_h}$ .
The problem of learning a region $r^*$ therefore reduces to identifying the corresponding labeling function $\ell_{r^*}$.
The objective here is to learn the region by querying the reference
of the form
    $q_{h}:= \mathbf{1}\curlybracket{\ell_{r^*}(h) = 1}$,
where $h \in \Hnd$ and $\mathbf{1}\curlybracket{\cdot}$ is the indicator function. 
Similar to the teaching setting, we assume that $\rgn^*$ is sampled uniformly at random. 
In the following, we show sample complexity results, i.e., on the minimal number of halfspace queries required to determine a target region , under the settings of \tt{active} and \tt{passive} learning. Specifically, we come up with a query selection procedure to achieve a tight bound for active learning as shown in \iftoggle{longversion}{\appref{appendix: active learning}}{the supplemental materials}.

\begin{theorem}\label{pairwise teaching bound}
Assume $\rgn$ $\sim$ $\mathcal{U}$ and that the underlying hyperplane arrangement of $\Hnd$ is in $d'$-relaxed general position. %Let $M_n$ denote a random variable for the number of queries that are requested in the query selection procedure, then $\mathbb{E}_{\mathcal{U}}[M_n] = \bigTheta{d'\log n}$, \tt{i.e.} 
Then, the average-case query complexity for actively learning a convex polytope is $\bigTheta{d'\log n}$,
and the worst-case query complexity is $\bigTheta{n}$.
\end{theorem}
%\paragraph{Passive learning} 
In \emph{passive learning} setting, %of a target region, 
the \tt{average} sample complexity is trivially lower bounded by $\bigOmega{n}$ since the learner gets a label uniformly at random. Thus, on average it requires $n$ samples to reconstruct the labels for all the halfspaces corresponding to the enclosing hyperplanes. Since there are $n$ hyperplanes $n$ samplings are sufficient to get all the labels which trivially give a $\cO(n)$ solution. Thus, it is not difficult to see that in the case of passive learning the average sample complexity is $\bigTheta{n}$. 
\looseness -1

%-----------Figures for general position definitions illustration
\begin{wrapfigure}{r}{0.16\textwidth}
\vspace{-10mm}
\centering
	\begin{subfigure}[b]{3pt}
	   \centering
		\includegraphics[width=.8\linewidth]{fig/3general.pdf}
		\vspace{-1mm}
		\caption{general}
		\label{fig:example.3general}
	\end{subfigure}
	\begin{subfigure}[b]{3pt}
	    \centering
		\includegraphics[width=.8\linewidth]{fig/2general.pdf}
		\vspace{-1mm}
		\caption{2-relaxed}
		\label{fig:example.2general}
	\end{subfigure}	
	\begin{subfigure}[b]{3pt}
	    \centering
		\includegraphics[width=.8\linewidth]{fig/1general.pdf}
		\vspace{-1mm}
		\caption{1-relaxed}
		\label{fig:example.1general}
	\end{subfigure}	
	\vspace{-6mm}
	\caption{relaxed general position}\label{fig:illu-relaxed-general}
\vspace{-8mm}	
\end{wrapfigure}

==> macros_alt.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}
% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
%\usepackage[nonatbib,preprint]{neurips_2020}
%\PassOptionsToPackage{numbers, compress}{natbib}\usepackage{neurips_2020}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[nonatbib]{neurips_2020}

%\usepackage{times}
\usepackage{savesym,multirow,xspace,enumitem,color}
\usepackage[dvipsnames]{xcolor}
%\usepackage{hyperref}
\usepackage[backref=page]{hyperref}
\hypersetup{
  citecolor = NavyBlue,
  colorlinks = true
  % linkbordercolor = {green},
}
\usepackage{backref}

%\usepackage[dvipsnames]{xcolor}
\usepackage[titletoc]{appendix}
%\usepackage[tight]{subfigure}
\usepackage{subcaption}
\usepackage{dsfont}
\usepackage{multicol}

\usepackage{wrapfig}


% toggle command
\usepackage{etoolbox}
%----------------Macros from colt
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage[final]{neurips_2018}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{verbatim}
\usepackage{amsmath,bm}
%\usepackage{algorithm}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{comment}
%\usepackage{algorithmicx}

%\usepackage[ruled]{algorithm}
%\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}

% algorithm2e package
%\usepackage[lined, boxed, ruled, commentsnumbered, noend]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
%\SetCommentSty{mycommfont}

\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\eqdef}{=\mathrel{\mathop:}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtoggle{showcomments}
\settoggle{showcomments}{true}


%\newcommand{\val}{{\text{val}}}
%\newcommand{\citet}[1]{\citeauthor{#1} (\citeyear{#1})}
\iftoggle{showcomments}{
\newcommand{\akash}[1]{{\textcolor{purple}{[{\bf Akash:} #1]}}}
\newcommand{\adish}[1]{{\textcolor{red}{[{\bf Adish:} #1]}}}
\newcommand{\yuxin}[1]{{\textcolor{ForestGreen}{[{\bf Yuxin:} #1]}}}
\newcommand{\yisong}[1]{{\textcolor{NavyBlue}{[{\bf Yisong:} #1]}}}
\newcommand{\annotate}[1]{{\textcolor{blue}{[{\bf Note:} #1]}}}
}
{
\newcommand{\akash}[1]{}
\newcommand{\adish}[1]{}
\newcommand{\yuxin}[1]{}
\newcommand{\yisong}[1]{}
\newcommand{\annotate}[1]{}
}

% % toggle command
% \usepackage{etoolbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\let\proof\relax
\let\endproof\relax
%\usepackage[lined, boxed, ruled, commentsnumbered,noend]{algorithm2e}
%, noend
\usepackage{xfrac}
\setitemize{noitemsep,topsep=1pt,parsep=1pt,partopsep=1pt, leftmargin=12pt}

%%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{fact}{Fact}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{assumption}{Assumption}
%\newtheorem{example}{Example}
%%%%%%%%%%%%%%%%%%%% NEW %%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{theorem}{Theorem}[section]
%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{assumption}{Assumption}%[section]
%\newtheorem{condition}{Condition}
\newtheorem{condition}[theorem]{Condition}

%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}[theorem]{Lemma}




\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
%\usepackage{mathtools}
\makeatother
\usepackage{caption}
\newcounter{copyrightbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\denselist}{
  % \itemsep -2pt\topsep-8pt\partopsep-8pt
  \itemsep -2pt\topsep-5pt\partopsep-5pt\itemindent-10pt
}
\newcommand{\Rd}{\mathbb{R}^d}


% % References
% ----------------------------------------------------------------
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{\text{Eq.}~(\ref{#1})}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\appref}[1]{Appendix \ref{#1}}
% \newcommand{\appref}[1]{the Appendix} % for short version of the paper
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\conref}[1]{Condition~\ref{#1}}
\newcommand{\assref}[1]{Assumption~\ref{#1}}
%\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\egref}[1]{Example~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
%\newcommand{\lineref}[1]{Line~\ref{#1}}


% Text conveniences
% ------------------------------------------------------------------------------
\newcommand{\cf}{\emph{c.f.}}

% Wrappers: Parens, brackets, etc
% -------------------------------------------------------------------------------
\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\parenb} [1] {\ensuremath{ \big( {#1} \big) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
\newcommand{\biggparen} [1] {\ensuremath{ \bigg( {#1} \bigg) }}
\newcommand{\Biggparen} [1] {\ensuremath{ \Bigg( {#1} \Bigg) }}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\tuple}[1]{\ensuremath{\left\langle #1 \right\rangle}}
%\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\curlybracket}[1]{\ensuremath{\left\{#1\right\}}}

\newcommand{\condcurlybracket}[2]{\ensuremath{\left\{#1\left\lvert\:#2\right.\right\}}}

% Functions and Functionals
% --------------------------------------------------------
\renewcommand{\Pr}[1]{\ensuremath{\mathbb{P}\left[#1\right] }}
\newcommand{\expct}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\expctover}[2]{\mathbb{E}_{#1}\!\left[#2\right]}
%\newcommand{\E}[1]{\ensuremath{\mathbb{E}\left[#1\right] }}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
%\newcommand{\argmax}{\operatorname{arg\,max}}
%\newcommand{\argmin}{\operatorname{arg\,min}}
\def \argmax {\mathop{\rm arg\,max}}
\def \argmin {\mathop{\rm arg\,min}}


% asymptotics
\newcommand{\littleO}[1]{\ensuremath{o\paren{#1}}}
\newcommand{\bigO}[1]{\ensuremath{\mathcal{O}\paren{#1}}}
\newcommand{\bigTheta}[1]{\ensuremath{\Theta\paren{#1}}}
\newcommand{\bigOmega}[1]{\ensuremath{\Omega\paren{#1}}}

\newcommand{\bigOTilde}[1]{\ensuremath{\tilde{O}\paren{#1}}}


% fundamental sets and objects
\newcommand{\NonNegativeReals}{\ensuremath{\mathbb{R}_{\ge 0}}}
\newcommand{\PositiveIntegers}{\ensuremath{\mathbb{Z^+}}}
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\nats}{\ensuremath{\mathbb{N}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\rationals}{\ensuremath{\mathbb{Q}}}
\newcommand{\distrib}[0]{\ensuremath{\mathcal{D}}}
\newcommand{\matroid}{\ensuremath{\mathcal{M}}}
\newcommand{\model}[0]{\ensuremath{\mathcal{M}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Caligraphic Vars
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cO}{{\mathcal{O}}}

\newcommand{\cL}{{\mathcal{L}}}

% Bold vars
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bff}{{\mathbf{f}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bZ}{{\mathbf{Z}}}


% \mathfrak caligraphgy
\newcommand{\ff}{{\boldsymbol{\mathfrak{F}}}}
\newcommand{\fr}{{\boldsymbol{\mathfrak{r}}}}

%d'-general position

\newcommand{\Hnd}{\boldsymbol{\mathcal{H}}_{n,d}}
\newcommand{\Hndp}{\boldsymbol{\mathcal{H}}_{(n),d}}
\newcommand{\Hndo}{\boldsymbol{\mathcal{H}}_{n-1,d-1}}
\newcommand{\xnd}{\boldsymbol{\mathcal{X}}_{n,d}}
\newcommand{\xndp}{\boldsymbol{\mathcal{X}}_{n,d}^{+}}
\newcommand{\xndn}{\boldsymbol{\mathcal{X}}_{n,d}^{-}}
\newcommand{\Hndd}{\boldsymbol{\mathcal{H}}_{n,d'}^{ind}}
\newcommand{\rnd}{\boldsymbol{\fr}\parenb{\cA(\Hnd)}}
\newcommand{\regionset}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\Hnd)}}
\newcommand{\regionpair}{\boldsymbol{\mathfrak{R}}\parenb{\mathcal{A}(\boldsymbol{\mathcal{H}}_{(n),d})}}
\renewcommand{\tt}[1]{\textit{#1}}
\newcommand{\rank}[1]{\textbf{rank}\parenb{#1}}
\newcommand{\lam}{\parenb{\mathbf{\Lambda}}}
\newcommand{\boldlam}{\mathbf{\boldsymbol{\Lambda}}}
\def\mathbi#1{\textbf{\em #1}}
\newcommand{\varstackrel}[3][T]{\stackrel{\raisebox{0.5ex}{\scriptsize#2}}{#3}}

%\newcommand{\boldlam}{\textLambda}
\def\BState{\State\hskip-\ALG@thistlm}

%Data space and Hypothesis space 
\newcommand{\data}{\textit{data space}}
\newcommand{\hypo}{\textit{hypothesis space}}
\newcommand{\wrt}{\mathrm{wrt}}
\newcommand{\gen}{{$d'$-\textit{relaxed general position}}}
\newcommand{\up}[1]{\Upsilon_{\mathrm{dual}}\parenb{#1}}
\newcommand{\upi}[1]{\Upsilon^{-1}_{\mathrm{dual}}\parenb{#1}}
\newcommand{\vari}[1]{\varphi^{-1}_{\mathrm{dual}}\parenb{#1}}
%\newcommand{\comment}[1]{}
%00000000000Macros for variables 
\newcommand{\h}{z}
\newcommand{\dt}{x}
\newcommand{\rgn}{r}
%\newcommand{}{y}


==> statement_of_broader_impact.tex <==
\section*{Broader Impact}
Our research will potentially impact sub-fields of ML and AI including active learning, passive learning, and machine teaching. Theoretically, our analysis of sufficiency and necessity of required number of examples to teach a target concept directly impacts how we design curriculum for education ranging from human learning to teaching intelligent agents for Medical, IT applications, etc. Since the analysis can greatly enhance our understanding of how we can teach efficiently, we can accelerate the spectrum of learning. Due to the conceptual/theoretical nature of this work, the ethical and societal implications are not applicable.
